LLaVA-3D: A Simple yet Effective Pathway to Empowering LMMs with 3D-awareness

Recent advancements in Large Multimodal Models (LMMs) have greatly enhanced their proficiency in 2D visual understanding tasks, enabling them to effectively process and understand images and videos. However, the development of LMMs with 3D scene understanding capabilities has been hindered by the lack of large-scale 3D vision-language datasets and powerful 3D encoders. In this paper, we introduce a simple yet effective framework called LLaVA-3D. Leveraging the strong 2D visual understanding priors from LLaVA, our LLaVA-3D efficiently adapts LLaVA for 3D scene understanding without compromising 2D understanding capabilities. To achieve this, we utilize the 3D position embeddings to enhance the 2D CLIP Patches with 3D spatial context information and construct 3D patches. By integrating the 3D position embeddings into 2D LMMs and employing joint 2D and 3D vision-language instruction tuning, we establish a unified architecture for both 2D visual understanding and 3D scene understanding. In contrast to previous 3D LMMs, LLaVA-3D supports decoding accurate 3D spatial perception outputs, e.g., 3D bounding boxes, directly from these 3D patches, without relying on the time-consuming off-the-shelf 3D segmentors. Experimental results show that LLaVA-3D converges 3.5x faster than existing 3D LMMs when trained on 3D vision-language datasets. Moreover, LLaVA-3D not only achieves state-of-the-art performance across various 3D tasks but also maintains comparable 2D visual understanding and vision-language conversation capabilities with LLaVA.

==> figures/convergene.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=0.85\linewidth]{imgs/convergence.png}
   \captionsetup{aboveskip=0pt}\captionsetup{belowskip=0pt}\caption{Loss curves for training the LLaVA-3D and Scene-LLM. Compared with adapting LLM to 3D formulation, lifting image-domain MLLM to 3D converges faster.} 
   \label{fig:convergence}
\end{figure}

==> figures/data_distribution.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{imgs/llava-3d-data-v2.png}
    \captionsetup{aboveskip=10pt}\captionsetup{belowskip=0pt}\caption{\textbf{LLaVA-3D-Instruct-1M.} The hybrid 2D and 3D Dataset Collection. Left: Distribution of data across categories, with the outer circle representing all categories and the inner circle illustrating data subset distribution. Right: Detailed dataset quantities.} 
   \label{fig:instruct_data}
\end{figure}

==> figures/demo1.tex <==
\begin{figure*}[t]
  \centering
   \includegraphics[width=0.9\linewidth]{imgs/demo1.png}
   \captionsetup{aboveskip=5pt}\captionsetup{belowskip=0pt}\caption{LLaVA-3D could perform 2D Click-based 3D dense captioning, generating the corresponding object caption and 3D bounding box.} 
   \label{fig:demo_1}
\end{figure*}

==> figures/demo2.tex <==
\begin{figure*}[t]
  \centering
   \includegraphics[width=1\linewidth]{imgs/demo2.png}
   \captionsetup{aboveskip=5pt}\captionsetup{belowskip=0pt}\caption{LLaVA-3D could perform 2D Click-based 3D question answering, now users could click on the 2D images and ask the question.} 
   \label{fig:demo_2}
\end{figure*}

==> figures/demo3.tex <==
\begin{figure*}[t]
  \centering
   \includegraphics[width=1\linewidth]{imgs/demo3.png}
   \captionsetup{aboveskip=5pt}\captionsetup{belowskip=0pt}\caption{LLaVA-3D exhibits powerful 3D visual grounding capability, enabling accurate 3D bounding boxes output.} 
   \label{fig:demo_3}
\end{figure*}

==> figures/model.tex <==
\begin{figure*}[t]
  \centering
   \includegraphics[width=\linewidth]{imgs/llava3d-architecture.png}
   \captionsetup{aboveskip=10pt}\captionsetup{belowskip=0pt}\caption{\textbf{LLaVA-3D Architecture.} Based on LLaVA, we directly add the corresponding 3D position embeddings to 2D patch visual tokens of multi-view images to construct the 3D Patches, then the 3D Patches will undergo 3D pooling and be sent into the projection layer of LLaVA to map into the LLM space and align with the LLM using 3D-visual-language data.} 
   \label{fig:method}
\end{figure*}

==> figures/new_teaser.tex <==
\begin{figure*}[!ht]
   \includegraphics[width=1\linewidth]{imgs/new_teaser_2.png}
    
    \caption{\textbf{Overview of LLaVA-3D.} The left block shows that compared with previous 3D LMMs, our LLaVA-3D achieves state-of-the-art performance across a wide range of 3D scene understanding benchmarks while maintaining a comparable performance on 2D multimodal benchmarks compared with LLaVA-Video. The middle block demonstrates that LLaVA-3D leverages 3D patches to endow the 2D LMMs with 3D spatial awareness, enabling it to perform various 3D vision-and-language tasks in the physical world. The right block highlights the significantly faster convergence and inference speeds of LLaVA-3D compared to existing 3D LMMs.} 
   \label{fig:new_teaser}
\end{figure*}

==> figures/performance.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{imgs/llava-3d-performance.png}
    \captionsetup{aboveskip=10pt}\captionsetup{belowskip=0pt}\caption{\textbf{LLaVA-3D} achieves SoTA on a broad range of 3D benchmarks, and maintains the comparable performance on various 2D benchmarks compared with LLaVA-1.5.} 
   \label{fig:performance_radio}
\end{figure}

==> figures/scaling_law.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{imgs/scaling-law.png}
    \captionsetup{aboveskip=5pt}\captionsetup{belowskip=0pt}\caption{Scaling laws under different sampling strategies. Both data sample and scene diversity matter when scaling up the training and more diverse scenes can
result in more significant improvement.} 
   \label{fig:scaling-law}
\end{figure}

==> figures/tasks.tex <==
\begin{figure*}[t]
  \centering
   \includegraphics[width=0.95\linewidth]{imgs/tasks_illustration_v2.png}
    \captionsetup{aboveskip=5pt}\captionsetup{belowskip=0pt}\caption{\textbf{LLaVA-3D} extends the capability of 2D LMMs to multi-modal 2D and 3D vision-language tasks with a unified model. For 2D V\&L tasks, the inputs of LLaVA-3D are only single or multi-view images, and for 3D V\&L tasks, apart from the multi-view images, the inputs should also contain the depth images and camera parameters.} 
   \label{fig:task}
\end{figure*}

==> figures/teaser.tex <==
\begin{figure*}[!ht]
   \includegraphics[width=1\linewidth]{imgs/llava-3d-teaser-combine-v2.png}
    
    \caption{\textbf{Overview of LLaVA-3D.} The left block shows that compared with previous 3D LMMs, our LLaVA-3D achieves state-of-the-art performance across a wide range of 3D benchmarks while maintaining a comparable performance on various 2D benchmarks compared with LLaVA-1.5. The middle block demonstrates that LLaVA-3D is built on the 2D LMM: LLaVA, and leverages 3D patches to endow it with 3D spatial awareness, enabling it to perform various 3D vision-and-language tasks in the physical world. The right block highlights the significantly faster convergence and inference speeds of LLaVA-3D compared to existing 3D LMMs.} 
   \label{fig:teaser}
\end{figure*}

==> figures/visualization.tex <==
\begin{figure*}[t]
  \centering
   \includegraphics[width=0.85\linewidth]{imgs/example.png}
    \captionsetup{aboveskip=5pt}\captionsetup{belowskip=0pt}\caption{\textbf{Qualitative Result of the LLaVA-3D}. Our model demonstrates superior capability in
understanding 3D spatial information.} 
   \label{fig:visualization}
\end{figure*}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Multimodal Large Language Models (MLLMs) have demonstrated remarkable proficiency in image comprehension when trained on large-scale image-text pairs.  For 3D vision area, the recent 3D-visual-language models also explore a similar pipeline to finetune LLMs on large-scale 3D-visual-language data.  However, considering the fact that: 1)  the size of currently collected 3D visual-language datasets is far behind the billion-scale image-text datasets used for training 2D Multimodal Language Learning Models (MLLMs). 2)  there are no available powerful pre-trained 3D encoders like CLIP ViT encoders for 2D images in 3D scenes. Thus, retraining 3D-visual-language models from scratch is data-inefficient and resource-heavy. Meanwhile, for the video-language models, facing similar data resources limitation, recent works [VideoLLaVA, PLLaVA, LLaVA-Next] try to adapt the pre-trained image-domain MLLMs (LLaVA) to video data by encoding multiple video frames into a sequence of features and directly feed them into image-domain MLLMs, achieving impressive video understanding ability. An intuitive question naturally arises: \textit{Can we adapt image-domain MLLMs to 3D scene understanding?}

Let’s review how to represent a 3D scene:  An agent is deployed to scan indoor environments with an RGB-D camera, generating a video sequence consisting of multiview RGB-D images with camera parameters (pose and intrinsic), and these sensed RGB-D frames can be post-processed into a single colored 3D point clouds through reconstruction. Currently,  3D scene understanding models uasually perform on the reconstructed 3D point clouds. However, such pipeline is perhaps inconsistent with the goals of embodied egent vision (and typical 2D vision). In other words, for the embodied agent, the 3D scene understanding can be regarded as a variant of ``video understanding''.  However, it's nontrival to directly follow the video-language model adpation paradigm to build 3D-visual-language model considering the different goals: video-language models aims to understand the temporal information to describe the video by simply processing the sequential image features frame-by-frame, while 3D visual-language models requires to understand 3D spatial information from the scene video. 

For a collected RGB-D video, each frame in the video represents the agent’s egocentric observation of the scene from a specific location and orientation, and all the observations from the agent could be aggregated into the holistic scene-level representation. Current image-domain MLLMs [LLaVA/GPT-4V] could perform partial scene observation understanding from one or multiple frame images, they lack the ability to figure each frame's observation spatial location in the 3D scene and achieve the cross observation consistency. 

To make LLM capable of understanding the 3D spatial information, we proposes \textbf{LLaVA-S}, lifing the LLaVA to 3D scene by explicitly injects the 3D position information into the image features. LLaVA-S can perform frame-level 2D and 3D understanding and scene-level 3D understnading, our contributions can be summarized as:

\begin{itemize}

    \item We are the first attempt to directly apply image-domain MLLMs to 3D scene understanding tasks by simply introducing 3D position embeddings to the visual features.
    % \item We introduce a 2D/3D joint-tuning method that could effectively keep the original 2D understanding ability of the image-domain MLLMs during 3D V\&L tasks fine-tuning.
    \item Our proposed model is the first MLLM capable of understanding both 2D images and 3D scenes at the same time, showing promising performance across various 2D/3D V\&L benchmarks.
    \item We conduct extensive experiments to demonstrate the superiority of the proposed model and achieve a new state-of-the-art across various 3D V\&L benchmarks while training on much less 3D V\&L datasets. 
\end{itemize}




==> sec/1_intro_v2.tex <==
\section{Introduction}
\label{sec:intro}

% background: LMM -> LMM with spatial intelligence
Recent Large Multi-modal Models (LMMs)~\misscite have shown impressive performance in understanding images and language instructions.
However, despite their strong perception and reasoning capabilities, they still mainly serve as assistants through daily interactions with us in the virtual world through images or videos \xihui{their abilities are limited to understanding 2D images and videos}, while lacking the ability to understand the \xihui{real} 3D world. To enable real applications in the physical world and further evolve new emerging capabilities through physical interaction, equipping them with 3D spatial intelligence is a necessity.

\input{figures/teaser}


% previous works: 3D+LLM is hard
% Built upon LLM, 3D-LLM & Scene-LLM takes multi-view images as input -> limitations, other related works?
% Built upon 2D LMM foundation, can it handle by itself? How can we build 3D capability on it?
One of the most important capabilities for spatial intelligence is to perceive and understand the 3D world. Similar to 2D LMMs, which aligns the 2D image features with LLM utilizing the large-scale 2D vision-language dataset,
%the natural way to achieve it is by integrating typical 3D representations, such as point clouds, directly into existing LMMs with 3D vision-language datasets for alignment~\misscite. \xihui{% 
a typical previous approach for building the 3D-LLMs is to inject the 3D features encoded from point cloud into Large Language Models (LLMs) and train the 3D-LLMs with 3D point cloud-language datasets.

However, in contrast to the large-scale image and video data, such 3D data is still significantly scarce, and there are no powerful pre-trained 3D encoders like CLIP ViT~\misscite in 2D \xihui{confusing grammar. Sentence is too long.} as the foundation, making this pathway difficult in the current circumstance.
Considering the raw observation of embodied agents in the real world is typically ego-centric multi-view images~\misscite \xihui{is this clear enough to describe the data representation?}, it is reasonable to build the 3D spatial foundation model with such input. There have been several works~\misscite built upon the LLM foundation exploring along this way, but suffering from complex and time-consuming 3D feature extraction processes utilizing 2D encoders.\footnote{Previous CLIP can only handle object-centric patches and the extracted 3D features are typically pixel-wise from segmentation priors.} A question arises: \textit{Can we directly build the 3D LLM upon the 2D LMMs trained on large-scale data, to utilize the 2D strong prior and avoid the challenging 3D encoders?}

% \xihui{The logic of this paragraph is not clear. Seems you want to discuss three things: (1) 3D data is less than  2D data, (2) 3D encoder is less powerful than 2D encoder, (3) 3D representation: point cloud v.s. multi-view images. It can be re-organized in this way: (1) briefly introduce how 2D LLMs work. (2) Some previous works investigate point cloud-based 3D-LLMs with a point cloud encoder and large language models. (3) However, the lack of 3D data and the inferior performance of 3D encoder limits the potential of this pathway. (4) In order to build a strong model for 3D understanding with limited 3D data, we need to make the best use of the strong prior from 2D LLMs trained on large-scale data. xxxx....}

% Our framework, how to make it, and its property
Given the recent progress in 2D LMMs, we devise a simple yet effective framework, LLaVA-3D, built upon the well-developed 2D LLaVA, to adapt it to understand the 3D world efficiently while retaining the original strong capabilities in 2D multi-modal perception and reasoning.
The key ingredient therein is a 3D representation, \emph{3D Patch}, that is proposed to connect 2D features in the 3D world for spatial understanding.
It is simply obtained by adding 3D position embeddings to 2D patch-wise features without any further complex processing.
Based on the original LLaVA framework, we first decorate 2D visual tokens as mentioned to derive the 3D patch features and then adopt various pooling strategies to handle the difficulty of compressing features given extensive input frames. By fine-tuning the model with existing 3D vision-language datasets, our model efficiently converges and gains 3D spatial understanding and grounding capabilities. Moreover, the model architecture unification allows LLaVA-3D to maintain the original strong 2D understanding and reasoning capabilities through joint instruction-tuning on 2D vision-and-language datasets.

% Fine-tuning the projection and LoRA layers of this framework with existing 3D vision-language datasets, this model can efficiently converge and do inference with learned spatial understanding capabilities, while maintaining the original 2D understanding and reasoning performance by joint-tuning on the 2D V\&L datasets.

% Experiments
Experiments demonstrate that Our LLaVA-3D achieves state-of-the-art performances on the 3D tasks and benchmarks: including 3D captioning, 3D question answering, and 3D grounding, while requiring significantly less training time and fewer epochs than existing 3D LMMs [LEO][LL3DA]. Meanwhile, by joint-tuning on 2D vision-language datasets, LLaVA-3D maintains strong 2D image understanding, reasoning, and conversation ability compared with the original LLaVA. 

% We conduct extensive experiments to demonstrate the superiority of our method on commonly used 3D vision-language benchmarks. LLaVA-3D achieves SOTA performance on 3D QA benchmark: 54.9\% and 27.9\% on SQA3D and ScanQA respectively, and comparable AP25 33.7\% on 3D grounding benchmark: ScanRefer. Besides, LLaVA-3D maintains strong 2D image understanding and reasoning ability compared with original 2D LLaVA.
% \tai{Need more results and highlights, please refer to other papers}


% Recent advancements in Large Multimodal Models (LMMs) have shown impressive abilities in understanding images when trained on large-scale image-text pairs. However, despite their strong communication and reasoning skills, these models lack grounding in the real 3D physical world, which is essential for an embodied agent to interact with the environment. Therefore, developing a robust and powerful 3D visual-language model could be the next step towards achieving Artificial General Intelligence (AGI).


% However, due to the fact that: 1)  the size of currently collected 3D visual-language datasets is far behind the billion-scale image-text datasets used for training 2D Language Multimodal Models (LMMs). 2) there are no available powerful pre-trained 3D encoders like CLIP ViT encoders for 2D images in the 3D scene, building a 3D-visual-language model from scratch is data-inefficient and resource-heavy. Recently many works [3D-LLM / Scene-LLM] tend to construct the 3D-visual-language model utilizing the pre-aligned 2D features (CLIP). Specifically, they extract pixel-wise CLIP features from each image, aggregate them into a 3D point set using depth and camera parameters to explicitly construct the 3D world, and then align the 3D point features with the LLM utilizing various 3D-visual-language data. However, this paradigm has some issues: 1) the 3D feature extraction process is very complex and time-consuming. 2) The data used in the alignment process is still limited to 3D visual-language datasets. On the other hand, for an embodied agent, a 3D scene could be depicted by multi-view images from different perspectives, where the visual correspondence and disparity could implicitly indicate the spatial information in the 3D world. An LMM trained on large-scale image/video-text datasets that can accept multiple images as input may can be used to understand the 3D world. However, an embodied agent must not only be capable of understanding the 3D world but also possess the ability to ground language in the physical world, which in turn allows the embodied agent to effectively comprehend and interact with their surroundings, which may require the explicit 3D world representation.

% To avoid the challenges of 3D scene feature extraction and achieve explicit 3D world understanding, in this paper, we propose LLaVA-3D, adapting the LLaVA architecture to understand the 3D world. We first explore whether a 2D LMM can truly understand the 3D scene through multi-view images, and then propose a simple but effective approach to empower 2D LMM with the explicit 3D world understanding and grounding ability by simply injecting the position information into the image features. Based on the same architecture, LLaVA-3D could preserve the learned information from large-scale image-text datasets and even enjoy the benefits through 2D \& 3D datasets joint training. Besides, we fully explore the pooling strategy to handle the dynamic and incremental 3D world while an embodied agent explores the 3D environment. Our contributions can be summarized as:

% \begin{itemize}

%     \item We fully explore the 3D understanding ability of current 2D LMM through various tasks.
%     \item We propose a simple but effective approach to empower the 2D LMM to explicitly understand the 3D world.
%     \item We conduct extensive experiments to demonstrate the superiority of the proposed model and achieve a new state-of-the-art across various 3D V\&L benchmarks. 
% \end{itemize}

% --------------original version------------------

% Recent advancements in Large Multimodal Models (LMMs) have shown impressive abilities in understanding images when trained on large-scale image-text pairs. However, despite their strong communication and reasoning skills, these models lack grounding in the real 3D physical world, which is essential for an embodied agent to interact with the environment. Therefore, developing a robust and powerful 3D visual-language model could be the next step towards achieving Artificial General Intelligence (AGI).


% However, due to the fact that: 1)  the size of currently collected 3D visual-language datasets is far behind the billion-scale image-text datasets used for training 2D Language Multimodal Models (LMMs). 2) there are no available powerful pre-trained 3D encoders like CLIP ViT encoders for 2D images in the 3D scene, building a 3D-visual-language model from scratch is data-inefficient and resource-heavy. Recently many works [3D-LLM / Scene-LLM] tend to construct the 3D-visual-language model utilizing the pre-aligned 2D features (CLIP). Specifically, they extract pixel-wise CLIP features from each image, aggregate them into a 3D point set using depth and camera parameters to explicitly construct the 3D world, and then align the 3D point features with the LLM utilizing various 3D-visual-language data. However, this paradigm has some issues: 1) the 3D feature extraction process is very complex and time-consuming. 2) The data used in the alignment process is still limited to 3D visual-language datasets. On the other hand, for an embodied agent, a 3D scene could be depicted by multi-view images from different perspectives, where the visual correspondence and disparity could implicitly indicate the spatial information in the 3D world. An LMM trained on large-scale image/video-text datasets that can accept multiple images as input may can be used to understand the 3D world. However, an embodied agent must not only be capable of understanding the 3D world but also possess the ability to ground language in the physical world, which in turn allows the embodied agent to effectively comprehend and interact with their surroundings, which may require the explicit 3D world representation.

% \input{figures/teaser}

% To avoid the challenges of 3D scene feature extraction and achieve explicit 3D world understanding, in this paper, we propose LLaVA-3D, adapting the LLaVA architecture to understand the 3D world. We first explore whether a 2D LMM can truly understand the 3D scene through multi-view images, and then propose a simple but effective approach to empower 2D LMM with the explicit 3D world understanding and grounding ability by simply injecting the position information into the image features. Based on the same architecture, LLaVA-3D could preserve the learned information from large-scale image-text datasets and even enjoy the benefits through 2D \& 3D datasets joint training. Besides, we fully explore the pooling strategy to handle the dynamic and incremental 3D world while an embodied agent explores the 3D environment. Our contributions can be summarized as:

% \begin{itemize}

%     \item We fully explore the 3D understanding ability of current 2D LMM through various tasks.
%     \item We propose a simple but effective approach to empower the 2D LMM to explicitly understand the 3D world.
%     \item We conduct extensive experiments to demonstrate the superiority of the proposed model and achieve a new state-of-the-art across various 3D V\&L benchmarks. 
% \end{itemize}



==> sec/2_related.tex <==
\section{Related Work}
\label{sec:formatting}

\paragraph{Singe-Image LMMs} Vision-language pre-training has obtained significant progress in the 2D image domain, starting from the single image LMM, such as [LLaVA][Mini-GPT][VILA][BLIP2]. [LLaVA] introduces a simple connection layer to align the 2D image with LLM and [BLIP2] uses a more Q-Former architecture to use the text feature to guide the 2D visual feature compression process. However, these methods can only accept a single 2D image as input and struggle to handle multiple image cases, which is essential for 3D scene understanding. Our LLaVA-3D is able to accept multiple images as input to comprehensively understand the whole scene.


\paragraph{Multi-Image LMMs} As LMMs have demonstrated superior performance across various single-image tasks, there has been increasing interest in extending their capabilities to multi-image understanding. In this domain, GPT-4V and Gemini has shown predominant performance compared with other open-source models. In fact, the video and 3D scene could be unified as mutli-image scenarios, represented as multi-frame images and multi-view images. The former has recently received significant attention and progress [Video-LLaVA][VideoChat][PLLaVA], while the latter is still unexplored [LLaVA-Next-Interleave]. By representing the 3D scene by multi-view images, the LMMs could enjoy the benefits from large-scale datasets (image-text and video-text datasets) and learn the implicit 3D world from multi-view images. Our LLaVA-3D starts from multi-view images and could further explicitly understand the 3D world and achieve 3D grounding and interaction ability.


\paragraph{Injecting 3D into LLMs} Recent advancements in Large Language Models (LLMs) have spurred research into expanding their capabilities to 3D environments, leading to the development of 3D LMMs. For 3D scene-level understanding, 3D LMMs need to process inputs such as point clouds [Chat-3D v2][LL3DA][LEO] or multi-view images [3D-LLM][[Scene-LLM] to perform tasks that require complex 3D spatial reasoning. An important distinction among these methods is how they construct the 3D scene representation. [LL3DA] directly uses a scene-level 3D point cloud encoder to extract the 3D scene representation. [LEO] and [Chat3D v2] first segment 3D objects from the scene point cloud using the off-the-shelf 3D instance segmentation model, and then independently extract 3D object features with object-level 3D encoders to represent the 3D scene. Starting from multi-view images, [3D-LLM] [Scene-LLM] obtain pixel-wise features from 2D foundation models (SAM, CLIP) across the multi-view images to form a 3D point-level scene representation. Different from the previous methods, our LLaVA-3D directly builds on the well-trained 2D LMM with multi-view images as input, enjoying the original 2D image understanding ability and further achieving powerful 3D spatial understanding ability.

% For 3D [3D-LLM][[Scene-LLM] align 3D point cloud features based on the CLIP with LLMs to perform tasks such as captioning, question answering. [LEO] performs exceptionally well as an embodied multi-modal generalist agent in perception, grounding, reasoning, planning, and action in 3D environments, demonstrating the potential of 3D-LLMs in comprehending and interacting with the physical world.  [LL3DA] takes in the 3D point cloud and responds to both textual instructions and visual prompts. Different from the aligning 3D points with LLM paradigm, our LLaVA-3D builds on the well-trained 2D LMM, enjoying the original semantic understanding ability and further achieves powerful 3D spatial understanding ability.

==> sec/3_model.tex <==
\section{Method}

In this section, we will introduce the architecture of LLaVA-3D.

\input{figures/model}

\subsection{Position-Aware Visual Token} After feeding a sequence of RGB-D video frames $X \in \mathbb{R}^{F \times C \times W \times H}$ into the CLIP-ViT model used in LLaVA, we can obtain the encoded vision feature $X_s \in \mathbb{R}^{F \times w \times h \times d}$, where each vision feature token corresponds one image patch. To inject the position information into the patch vision tokens, we backproject the vision tokens to 3D by lifting each feature vector to a corresponding 3D position $P \in \mathbb{R}^{F \times w \times h \times 3}$, using nearest neighbor depth and known camera intrinsic and extrinsic parameters. Then we consider to encode the XYZ coordinates of the visual tokens with an MLP as the visual token position embeddings, and add the position embeddings to the visual tokens to obtain the updated position-aware visual tokens $X' \in \mathbb{R}^{F \times w \times h \times d}$.

\subsection{Visual Token Pooling} Considering the need for 3D spatial information and the prohibitive costs associated with processing long RGB-D video inputs to MLLMs, such as large scene or robot navigation, similar to video-language model, pooling offers a straightforward and effective solution to meet both requirements. By pooling the vision tokens, we can obtain manageable token lengths for the LLM. However, different from video-language model, the visual tokens should be pooled according to their 3D position to maintain the need for dense 3D visual information. We explore
two different different parameter-free pooling strategies:

\paragraph{Voxelization Pooling} voxelizes the position-aware visual tokens, where the 3D space is discretized into a volumetric grid. In each occupied voxel, the visual tokens and XYZ coordinates undergo mean pooling to generate updated sets of voxel visual tokens and their corresponding spatial locations. Only the updated visual tokens from occupied voxels are fed into the LLM, which means the number of visual tokens are variable for different scenes.

\paragraph{FPS Pooling} Farthest Point Sampling (FPS) is a widely used technique that allows for the uniform selection of points from a point cloud. We can use FPS to sample the visual tokens from frames to a fixed number of tokens while ensuring that the sampled tokens cover the entire structure of the original scene by selecting the farthest points.


\subsection{Visual Language Alignment} The position-aware visual tokens will be mapped into LLM space by the projection layer in LLaVA to perform visual langaugae alignment. Overall, we only need to add a 3D position embedding layer to LLaVA to adapt it to 3D world understanding.













==> sec/4_align.tex <==
\section{Training}

To leverage the 2D priors from 2D LMMs, we train our LLaVA-3D model based on the pre-trained LLaVA-1.5. Due to the scarcity of 3D scene-language data, our training procedure comprises two stages for different training targets.

\vspace{3pt}
\noindent\textbf{Stage 1: 3D Patch Language Alignment.} During the first training stage, we use the region-level and scene-level caption data that describe spatial relationships among 3D objects to align the 3D patches with the LLM for enhanced 3D spatial comprehension. At this stage, the input multi-view images used are selected from sequences that correspond to specific regions or entire scenes. We freeze the vision encoder and LLM and only train the projection layer and 3D position embedding layer for efficient alignment. Since 3D patches are derived from CLIP features augmented with 3D positional information, the alignment between 3D Patch and LLM converges rapidly.

%In this stage, we further align the 3D patches and LLM from the 3D spatial understanding perspective, empowering LLM to understand the 3D position information contained in the 3D Patches. We use 3D region and scene caption datasets to train the projection layer, allowing efficient alignment and keeping the LLM frozen. Each scene caption could cover the object entities, 3D object spatial relationship, and the overall scene layouts in the 3D scene.\tai{How to align? What to fix and what to tune?}

% Besides, We hope that the visual token, even when explicitly injected with position embedding, still retains LLaVA’s inherent 2D image understanding ability. Therefore, we used LLMs to generate 3D frame-language data (frame-based caption) to train the position embedding layer and the project layer. We utilize 3D frame-language data under two coordinate systems: camera and world coordinates, to ensure that the model comprehends perspectives from both egocentric and scene-centric viewpoints.

\input{figures/data_distribution}

\vspace{3pt}
\noindent\textbf{Stage 2: Task Instruction Tuning.} 
During the instruction-tuning stage, LLaVA-3D is optimized to respond to complex 3D V\&L tasks and maintain its inherent 2D image reasoning and instruction-following capabilities. To facilitate this capability, we collect the \textbf{LLaVA-3D-Instruct-1M} dataset, a hybrid collection of 2D and 3D data specifically tailored for instruction tuning. The overall distribution of the dataset collection is shown in Fig~\ref{fig:instruct_data}, more details about the instructional tuning datasets are listed in the supplementary material. The 2D Data of LLaVA-3D-Instruct-1M is derived from existing LLaVA-1.5 instruction tuning data, ensuring the preservation of 2D image comprehension and conversation abilities. When tuning with 2D data, we keep the vision encoder frozen and jointly train the projection layer and LLM. The 3D Data of LLaVA-3D-Instruct-1M, on the other hand, comprises data from diverse 3D QA, 3D dense captioning, and 3D grounding tasks. During the 3D data instruction tuning, the 3D position embedding layer will be added to jointly train with the other modules. Additionally, for tasks where the instruction contains 3D coordinate information or requires 3D bounding box outputs, the corresponding encoding and decoding modules will be trained together. During instruction tuning, the 3D data pathway includes the 3D position embeddings and 3D patches, while the 2D data pathway is the original LLaVA. All modules except for the 3D position embeddings to construct 3D patches are shared across 2D and 3D data. This training setup ensures that LLaVA-3D is capable of processing both 2D and 3D visual tokens effectively, and is adaptive to various task formulations.


% We keep the vision frozen and jointly train the 3D position embedding layer, projection layer, and LLM together. We 3D QA, 3D dense caption, and 3D grounding data from different sources. For tasks where the instruction contains 3D position information or requires 3D bounding box outputs, the corresponding modules will be trained together. Besides, we aim to retain LLaVA’s inherent 2D image understanding ability as much as possible during the instruction-tuning stage. Therefore, we collect a new instruction tuning dataset \textbf{OmniDim}, a mixture of 2D and 3D data and conduct \textit{2D/3D V\&L tasks joint tuning} in this stage, and the details about the instruction tuning datasets refer to the appendix. The only difference in the instruction tuning for 2D and 3D tasks is whether the visual tokens used for LLM are 2D patches or 3D patches.

==> sec/5_exp.tex <==
\section{Experiments}

% \input{figures/performance}

\begin{table}[t]
\centering
\caption{\textbf{Quantitative comparison with SOTA models on various 3D QA tasks}. ``C'' stands for ``CIDEr'', ``B-4'' for ``BLEU-4'', ``M'' for ``METEOR'', ``R'' for ``ROUGE'', and ``EM@1'' for top-1 exact match. \textcolor{gray}{Gray} indicates evaluation results with refined exact-match protocol.}
\vspace{0.1em}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccccc}
    \toprule
     & \multicolumn{5}{c}{ScanQA (val)} & SQA3D (test) \\
     \cmidrule(lr){2-6} \cmidrule(lr){7-7}
      & C & B-4 & M & R & EM@1 & EM@1\\
    \midrule
    \multicolumn{1}{l}{\small\textbf{\textit{Task-specific models}}} \\
    Scan2Cap~\cite{scan2cap} & - & - & - & - & - & \hspace{2pt} 41.0$^\dagger$ \\
    ScanRefer+MCAN~\cite{scanrefer_mcan} & 55.4 & 7.9 & 11.5 & 30.0 & 18.6 & - \\
    ClipBERT~\cite{clipbert} & - & - & - & - & - & 43.3 \\
    ScanQA~\cite{scanqa} & 64.9 & 10.1 & 13.1 & 33.3 & 21.1 & 47.2 \\
    3D-VisTA~\cite{3d-vista} & 69.6 & 10.4 & 13.9 & 35.7 & 22.4 & 48.5 \\
    \midrule
    \multicolumn{1}{l}{\small\textit{\textbf{Task-specific fine-tuned 3D LMMs}}} \\
    3D-LLM (FlanT5)~\cite{3dllm} & 69.4 & 12.0 & 14.5 & 35.7 & 20.5 \\
    LL3DA~\cite{llava} & 76.8 & 13.5 & 15.9 & 37.3 & -  \\
    Chat-3D v2~\cite{chat3d-v2} & 87.6 & 14.0 & - & - & - & 54.7\\
    LEO~\cite{leo} & \textbf{101.4} & 13.2 & 20.0 & 49.2 & 24.5 \textcolor{gray}{(47.6)} & 50.0 \textcolor{gray}
    {(52.4)}  \\
    Scene-LLM ~\cite{scene-llm} & 80 & 12.0 & 16.6 & 40.0 & \textbf{27.2}  & 54.2\\
    \midrule
    \multicolumn{1}{l}{\small\textit{\textbf{Zero-shot 2D LMMs}}} \\
    VideoChat2~\cite{videochatv2} & 49.2 & 9.6 & 9.5 & 28.2 & 19.2 & 37.3 \\
    LLaVA-NeXT-Video~\cite{llava-onevision} & 46.2 & 9.8 & 9.1 & 27.8 & 18.7 & 34.2 \\
    GPT-4V & 59.6 & - & 13.5 & 33.4 & - & - \\
    Gemini & 68.3 & - & 11.3 & 35.4 & - & - \\
    Claude & 57.7 & - & 10.0 & 29.3 & - & - \\
    \midrule
    \rowcolor{gray!20} LLaVA-3D & 91.7 & 
    \textbf{14.5} & \textbf{20.7} & \textbf{50.1} & 27.0 \textcolor{gray}{(45.0)} & \textbf{55.6} \textbf{\textcolor{gray}
    {(57.6)}}\\
    \bottomrule
\end{tabular}
}
\label{tab:scanqa_sqa3d}
\end{table}

\begin{table*}
\centering
\caption{\textbf{Quantitative comparison on MMScan QA benchmark}. ``ST'' stands for Single-target, ``attr'' for attribute, ``OO'' for Object-Object, and ``OR'' for Object Region.``S.-BERT'', ``B-1'', ``B-4'', ``R.-L.'', ``MET.'' represents ``Sentence-BERT", ``BLEU-1'', ``BLEU-4'', ``ROUGE-L'', ``METEOR'', respectively. Here, we report the top-1 exact match with (the refined exact-match protocol results) for ``EM@1''.}
\resizebox{\textwidth}{!}
{
    \begin{tabular}{c|c|c|cc|ccc|c|>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{EFEFEF}}c|>{\columncolor[HTML]{EFEFEF}}c>{\columncolor[HTML]{EFEFEF}}c>{\columncolor[HTML]{EFEFEF}}c>{\columncolor[HTML]{EFEFEF}}c>{\columncolor[HTML]{EFEFEF}}c}
    \toprule
     \multirow{2}*{Methods} & \multirow{2}*{Setting} & \multirow{2}*{Overall} & \multicolumn{2}{c|}{Single-target} & \multicolumn{3}{c|}{Inter-target} &\multirow{2}*{Advanced} & \multicolumn{2}{>{\columncolor[HTML]{EFEFEF}}c|}{Data-driven Metrics} & \multicolumn{5}{>{\columncolor[HTML]{EFEFEF}}c}{Traditional Metrics}\\
    \cline{4-8}\cline{10-16}
    ~ & ~ & ~ & ST-attr & ST-space & OO-attr & OO-space & OR & ~ & SimCSE & S.-BERT & B-1. & B-4. & R.-L & MET. & EM@1 \\
    \hline
    3D-LLM~\cite{3dllm} & \multirow{4}*{Zero-Shot} & 28.6  & 37.8 & 18.8 & 13.7 & 26.3 & 15.4 & 20.8 &40.4 & 40.3 & 13.4 & 1.5 & 17.3 & 6.0 & 6.2 (19.6) \\
    Chat3D-v2~\cite{chat3d-v2} & ~ & 27.9 & 38.1 & 18.3 & 9.3 & 22.4 & 13.5 & 25.4 &45.4 & 46.3 & 18.0 & 3.0 & 22.9 & 7.5 & 10.2 (19.6) \\
    LL3DA~\cite{ll3da} & ~ & 15.8 & 15.5 & 14.7 & 14.2 & 25.2 & 4.3 & 6.4  & 40.7 & 43.6 & 5.4 & 2.1 & 16.4 & 4.4 & 8.3 (19.4) \\
    LEO~\cite{leo} & ~ & 22.2 & 28.9 & 17.6 & 18.1 & 20.4 & 15.0 & 16.3 &40.4 & 41.0 & 11.0 & 0.7 & 17.1 & 4.9 & 9.6 (18.7) \\
    \hline
    LL3DA~\cite{ll3da} & \multirow{2}*{Fine-tuning} & 38.5 & 40.4 & 46.2 & 14.7 & 47.1 & 26.4 & 7.1 & 65.3 & 67.0 & 26.4 & 8.5 & 44.3 & 14.7 & 30.2 (37.6)\\
    LEO~\cite{leo} & ~ & 47.8 & 55.5 & 49.5 & \textbf{36.1} & 45.6 & 32.1 & 38.4 & 71.2 & 72.2 & 32.0 & 12.5 &  52.1 & 17.7  & 36.6 (44.5)\\
    \hline
    LLaVA-3D & Generalist & \textbf{52.3} & \textbf{61.2} & \textbf{54.4} & 28.7 & \textbf{61.2} & \textbf{44.5} & \textbf{43.6} & \textbf{74.6} & \textbf{76.3} & \textbf{38.7} &\textbf{13.1}	&\textbf{55.5} &\textbf{19.5}	&\textbf{45.2 (51.4)} \\
    % \multirow{3}*{LLaVA-3D} & {1/10 Fine-tuning} & 48.1 & - & - & - & - & - & - & 70.6 & 71.7 & 36.8 &11.2	&51.7 &17.9	&40.2 (46.2) \\
    % & {1/4 Fine-tuning} & 53.0  & - & - & - & - & - & - &73.7 &76.3	&38.7	&12.2	&55.5	&19.5	&44.2 (51.4)\\
    % & {1/2 Fine-tuning} & \textbf{54.6} & - & - & - & - & - & - &74.1 &76.9	&39.2 &12.7 &56.1	&19.9 &\textbf{45.4} (52.1) \\
    \bottomrule
    \end{tabular}
}
\vspace{-1.5ex}
\label{tab:mmscan}
\end{table*}

\begin{table}
\centering
\caption{\textbf{Quantitative comparison with SOTA models on OpenEQA benchmark.}}
\resizebox{0.55\linewidth}{!}{
\begin{tabular}{c|c|c}
      \toprule
      Models & Frame & Accuracy \\
      \midrule
      LLaMA2~\cite{touvron2023llama} & 0 & 28.3 \\
      GPT-4~\cite{gpt-4} & 0 & 33.5 \\
      Claude3 & 20 & 36.3 \\
      Gemini-Pro~\cite{gemini} & 15 & 44.9 \\
      GPT-4V~\cite{gpt-4} & 15 & 54.6 \\
      GPT-4V~\cite{gpt-4} & 50 & 55.3 \\
      Human & Full & 86.8 \\
      \midrule
      \rowcolor{gray!20} LLaVA-3D & 20 & 51.2\\
      \bottomrule
    \end{tabular}
}
\label{tab:openeqa_results}
\end{table}


In this section, we conduct extensive evaluations to examine the capabilities of LLaVA-3D. We compare our model’s 3D scene understanding (Sec.~\ref{sec:qa_results},~\ref{sec:dc_results},~\ref{sec:vg_results}) and 2D image understanding (Sec.~\ref{sec:2d_benchmark}) capability with previous methods. Then we thoroughly analyze the effectiveness of the components and designs of our LLaVA-3D (Sec.~\ref{sec:arch_analysis},~\ref{sec:ablation}).

% \subsection{Implementation Details}
% \label{sec:exp_settings}

% LLaVA-3D is built upon the LLaVA-1.5-7B, utilizing their pre-trained weights from the HuggingFace library. For 3D tasks, we add the 3D position embeddings to the 2D patch visual tokens, and utilize the voxelization pooling strategy to reduce 3D patch number before passing the input visual tokens to the projection layer and LLM. The number of views $V$ is set to 20 and voxel size is set to 0.2m. Due to the LLM context length limitation, the maximum number of 3D patch tokens after 3D-aware pooling is set to 3096. For 2D tasks, LLaVA-3D functions the same as LLaVA. All experiments are conducted on 8 × 80G A100 GPUs. We train our model for 1 epoch with a learning rate of 1e-3 and a batch size of 32 in stage 1, and fine-tune on the collected LLaVA-3D-Instruct-1M dataset, with a learning rate of 2e-5 and a batch size of 16 in stage 2.


\subsection{Evaluation on 3D Question Answering}
\label{sec:qa_results}

3D Question Answering requires a model to generate responses to the natural language questions in a 3D scene. In this section, we validate LLaVA-3D performance on various 3D question answering benchmarks: ScanQA~\cite{scanqa}, SQA3D~\cite{sqa3d}, MMScan QA~\cite{mmscan}, and OpenEQA~\cite{openeqa}.

\vspace{3pt}
\noindent\textbf{Spatial Understanding with ScanQA and SQA3D.} ScanQA and SQA3D are both built on the ScanNet dataset. The ScanQA dataset consists of 41363 questions about 800 scenes, including 32337 unique questions. SQA3D comprises 20.4k descriptions of 6.8k unique situations collected from 650 ScanNet scenes and 33.4k questions about these situations. Questions in ScanQA require basic recognition and 3D reasoning capabilities, and SQA3D further incorporates situation understanding and situated reasoning into embodied 3D scene understanding. 
% Following prior works, we adopt BLEU scores, METEOR, ROUHE-L, CIDEr and EM (“exact match”) as our evaluation metrics for ScanQA and EM for SQA3D respectively. 
As shown in Tab.~\ref{tab:scanqa_sqa3d}, current 2D LMMs fail to achieve competitive performance with the latest 3D LMMs, which might be attributed to the lack of explicit 3D representation. Besides, compared with the 3D LMMs that need to be further fine-tuned on the corresponding datasets, our LLaVA-3D could perform as a generalist and achieve the SOTA performance on these benchmarks.

% MMScan covers 5.2k scans from ScanNet, 3RScan,
% and Matterport3D, and focuses on object-related 3D question answering. OpenEQA is the first open-vocabulary
% benchmark dataset for EQA supporting both episodic memory and active exploration use cases. For quantitative comparisons in ScanQA and SQA3D, we include both task-specific approaches and generalist models: the state-of-the-art specialists in 3D QA; and task-specific fine-tuned generalist models like 3D-VisTA, 3D-LLM, LL3DA, Chat-3D v2, LEO and Scene-LLM. Besides, we also test the video LMMs trained on videos for comparison, to validate whether they could implicitly learn 3D structure information through visual correspondence among images, as illustrated in Tab~\ref{tab:question-answering}. Our model achieved excellent results on the MMScan QA benchmark. Even when trained on only one-tenth of the dataset, our model managed to achieve state-of-the-art (SOTA) results. Furthermore, as the amount of data increases, the performance of the model continues to improve. 
\vspace{3pt}
\noindent\textbf{Coordinate Spatial Understanding with MMScan QA.} MMScan QA includes 5.2k scans from ScanNet, 3RScan, and Matterport3D, along with 116k training questions and 29k validation questions. These questions span existential inquiries, attribute understanding, and more advanced queries. Unlike ScanQA and SQA3D, some MMScan QA questions require 3D reasoning based on object coordinates rather than relying solely on text descriptions, demanding the model capable of understanding 3D coordinates information. 
%Under the GPT-4 evaluation, all data samples are classified into one of the following sub-categories: \{ST-attr, ST-space, OO-attr, OO-space, OR\}, and a minor part of QA samples are chosen for advanced understanding and reasoning, such as situated QA related to everyday life.%
We present the results under GPT-4 evaluation, data-driven metrics, and traditional metrics respectively in Tab.~\ref{tab:mmscan}. Our LLaVA-3D achieves significantly better performance compared to LL3DA and LEO which are further fine-tuned on full MMScan QA. The results highlight the training efficiency of LLaVA-3D and its strong 3D understanding ability to serve as the generalist model.

\vspace{3pt}
\noindent\textbf{Embodied Question Answering with OpenEQA.} OpenEQA is the first open-vocabulary benchmark designed for spatial understanding and embodied reasoning in embodied question answering. It features an automated evaluation protocol powered by LLMs, which shows strong alignment with human judgment. Our evaluations are conducted using the EM-EQA data split of OpenEQA, which includes over 1,600 high-quality, human-generated questions from diverse real-world environments. 
% In EM-EQA, the model is required to generate a textual answer to a question based on an episode history, consisting of posed RGB-D images. 
The results in Tab.~\ref{tab:openeqa_results} demonstrate that LLaVA-3D surpasses Claude3 and Gemini-Pro, and achieves comparable performance with powerful GPT-4V on this benchmark with significantly fewer model parameters.

% Besides, to further validate the 3D understanding ability, we found that current LMMs struggle with two complex tasks: object counting and spatial understanding. In particular, we compared the performance of the model on these two types of questions. \chenming{More detailed results analysis}

% \begin{table*}
% \centering
% \caption{\textbf{Quantitative comparison with SOTA models on various 3D QA tasks}. ``C'' stands for ``CIDEr'', ``B-4'' for ``BLEU-4'', ``M'' for ``METEOR'', ``R'' for ``ROUGE'', ``Sim'' for sentence similarity, and ``EM@1'' for top-1 exact match. \textcolor{gray}{Gray} indicates evaluation results with refined exact-match protocol.}
% \vspace{0.1em}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccccccccccc}
%     \toprule
%      & \multicolumn{5}{c}{OpenEQA} & \multicolumn{5}{c}{ScanQA (val)} & SQA3D (test) \\
%      \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-12}
%      & EM-EQA(ScanNet) & EM-EQA(HM3D) & EM-EQA(ALL) & A-EQA(HM3D) & A-EQA(HM3D) & C & B-4 & M & R & EM@1 & EM@1 \\
%     \midrule
%     \multicolumn{1}{l}{\small\textbf{\textit{Task-specific models}}} \\
%     Scan2Cap & - & - & - & - & - & - & - & - & - & - & \hspace{2pt} 41.0$^\dagger$ \\
%     3DJCG & - & - & - & - & - & - & - & - & - & - & - \\
%     Vote2Cap-DETR & - & - & - & - & - & - & - & - & - & - & - \\
%     ScanRefer+MCAN & - & - & - & - & - & 55.4 & 7.9 & 11.5 & 30.0 & 18.6 & - \\
%     ClipBERT & - & - & - & - & - & - & - & - & - & - & 43.3 \\
%     ScanQA & - & - & - & - & - & 64.9 & 10.1 & 13.1 & 33.3 & 21.1 & 47.2 \\
%     \midrule
%     \multicolumn{1}{l}{\small\textit{\textbf{Task-specific fine-tuned 3D LLMs}}} \\
%     3D-VisTA & 66.9 & 34.0 & 27.1 & 54.3 & 53.8 & 69.6 & 10.4 & 13.9 & 35.7 & 22.4 & 48.5 \\
%     3D-LLM (FlanT5) & - & - & - & - & - & 69.4 & 12.0 & 14.5 & 35.7 & 20.5 & - \\
%     LL3DA & - & - & - & - & - & 76.8 & 13.5 & 15.8 & 37.1 & - & - \\
%     Chat-3D v2 & - & - & - & - & - & 87.6 & 14.0 & - & - & - & 54.7 \\
%     LEO & 72.4 & 38.2 & 27.9 & 58.1 & 55.3 & \textbf{101.4} & 13.2 & 20.0 & 49.2 & 24.5 \textcolor{gray}{(47.6)} & 50.0 \textcolor{gray}
%     {(52.4)}\\
%     Scene-LLM & - & - & - & - & - & 80 & 12.0 & 16.6 & 40.0 & 27.2  & 54.2 \\
%     \midrule
%     \multicolumn{1}{l}{\small\textit{\textbf{Socratic LLMs}}} \\
%     GPT-4 w/ LLaVA-1.5 &45.4±1.3 &40.0±1.8 &43.6±1.1 &38.1±1.8 &7.0±0.4 & - & - & - & - & - & - \\
%     GPT-4 w/ CG &37.8±1.3 &34.0±1.7 &36.5±1.0 &34.4±1.8 &6.5±0.4 & - & - & - & - & - & - \\
%     \midrule
%     \multicolumn{1}{l}{\small\textit{\textbf{Multi-frame VLMs}}} \\
%     GPT-4V &57.4±1.3 &51.3±1.8 &55.3±1.1 &41.8±3.2∗ &7.5±0.6∗ & - & - & - & - & - & - \\
%     \midrule
%     LLaVA-3D & \textbf{58.3} & \textbf{52.1} & \textbf{58.2} & - & - & 90.1 & 
%     \textbf{16.2} & \textbf{17.6} & \textbf{49.4} & \textbf{27.9 \textcolor{gray}
%     {(49.2)}} & 54.9 \textbf{\textcolor{gray}
%     {(58.9)}}\\
%     \bottomrule
% \end{tabular}
% }
% \label{tab:vl_results}
% \end{table*}


% \begin{table}
% \centering
% \caption{\textbf{Quantitative comparison with SOTA models on OpenEQA benchmark}}
% \resizebox{0.65\linewidth}{!}{
% \begin{tabular}{c|c|c}
%       \toprule
%       Models & Frame & Accuracy \\
%       \midrule
%       LLaMA2~\cite{touvron2023llama} & 0 & 28.3 \\
%       GPT-4~\cite{gpt-4} & 0 & 33.5 \\
%       Claude3 & 20 & 36.3 \\
%       Gemini-Pro~\cite{gemini} & 15 & 44.9 \\
%       GPT-4V~\cite{gpt-4} & 15 & 54.6 \\
%       GPT-4V~\cite{gpt-4} & 50 & 55.3 \\
%       Human & Full & 86.8 \\
%       \midrule
%       \rowcolor{gray!20} LLaVA-3D & 20 & 51.2\\
%       \bottomrule
%     \end{tabular}
% }
% \label{tab:openeqa_results}
% \end{table}

% \begin{table}
% \centering
% \caption{\textbf{Quantitative comparison with SOTA models on OpenEQA benchmark}}
% \vspace{0.1em}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccc}
%     \toprule
%      & \multicolumn{3}{c}{OpenEQA} \\
%      \cmidrule(lr){2-4}
%      & EM-EQA(ScanNet) & EM-EQA(HM3D) & EM-EQA(ALL) \\
%     \midrule
%     \multicolumn{1}{l}{\small\textit{\textbf{Socratic LLMs}}} \\
%     GPT-4 w/ LLaVA-1.5 &45.4±1.3 &40.0±1.8 &43.6±1.1 \\
%     GPT-4 w/ CG &37.8±1.3 &34.0±1.7 &36.5±1.0 \\
%     GPT-4 w/ SVM &40.9±1.3 &35.0±1.8 &38.9±1.0 \\
%     LLaMA-2 w/ SVM &36.0±1.3 &30.9±1.8 &34.3±1.0  \\
%     \midrule
%     \multicolumn{1}{l}{\small\textit{\textbf{Multi-frame VLMs}}} \\
%     GPT-4V &57.4±1.3 &51.3±1.8 &55.3±1.1  \\
%     \midrule
%     LLaVA-3D & \textbf{58.3} & \textbf{52.1} & \textbf{56.2} \\
%     \bottomrule
% \end{tabular}
% }
% \label{tab:openeqa_results}
% \end{table}

\begin{table}[t]
    \caption{
        \textbf{Quantitative Comparisons with SOTA models for 3D Dense Captioning on Scan2Cap.} The n-gram metrics for Scan2Cap are governed by IoU@0.5.
    }
    \label{tab:benchmark-3d-dense-cap}
    \centering
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    & \multicolumn{4}{c}{Scan2Cap (Val)} \\ 
    \cline{2-5}  
                            & C@0.5$\uparrow$ & B-4@0.5$\uparrow$ & M@0.5$\uparrow$ & R@0.5$\uparrow$ \\ \hline
    Scan2Cap~\cite{scan2cap}                & 39.1           & 23.3             & 22.0           & 44.8      \\
    % MORE~\cite{more}              &  & 40.94           & 22.93             & 21.66           & 44.42          \\
    % SpaCap3D~\cite{spacap3d}             &  & 44.02           & 25.26             & 22.33           & 45.36          \\
    % % REMAN                  &  & 45.00           & 26.31             & 22.67           & 46.96           \\
    % D3Net~\cite{d3net}                  &  & 46.07           & 30.29             & 24.35           & 51.67         \\
    % % Contextual              &  & 46.11           & 25.47             & 22.64           & 45.96            \\
    % UniT3D~\cite{unit3d}                  &  & 46.69           & 27.22             & 21.91           & 45.98        \\
    % 3DJCG~\cite{3djcg}                 &  & 49.48           & 31.03             & 24.22           & 50.80       \\
    3D-VLP~\cite{3dvlp}              & 55.0           & 32.3             & 24.8           & 51.5          \\
    3D-VisTA~\cite{3d-vista}        & 61.6          & 34.1           & 26.8         & 55.0     \\
    Vote2Cap-DETR~\cite{vote2cap-detr}       & 61.8           & 34.5            & 26.2          & 54.4         \\
    % 
    LL3DA~\cite{ll3da}          & 65.2            & 36.8      & 26.0          & 55.0                  \\
    LEO~\cite{leo}    &72.4 &38.2 &27.9 &58.1 \\
    % Chat-Scene~\cite{chatscene}  &77.1 &36.5 &- &- \\
    \rowcolor{gray!20} LLaVA-3D  &\textbf{79.2} & \textbf{41.1} &\textbf{30.2}  & \textbf{63.4} \\
    \bottomrule
    \end{tabular}
    }
    \label{exp:comparison_on_scanrefer}
\end{table}

\begin{table}
\centering
\caption{\textbf{Quantitative comparison with SOTA models on the MMScan Captioning benchmark.}}
\resizebox{\linewidth}{!}
{
\begin{tabular}{c|c|cccccc|c}
\toprule
\multirow{1}{*}{model} & \multicolumn{1}{c|}{Evaluator}
& \multicolumn{1}{c}{Type} & \multicolumn{1}{c}{Color} & Shape & Position & Function & Design & \multicolumn{1}{c}{Overall} \\ \hline
LL3DA~\cite{ll3da} & GPT  & 10.0 & 26.3 & 40.6  & 38.9 & 67.5 & 21.7 & 33.6 \\
LEO~\cite{leo}  & GPT  & 34.9 & 29.7 & 63.0  & 63.7 & 75.0 & 42.7 & 51.3 \\
\rowcolor{gray!20} LLaVA-3D & GPT & \textbf{39.9} & \textbf{79.2} & \textbf{89.1} & \textbf{82.2} & \textbf{94.1} & \textbf{88.0} & \textbf{78.8} \\
\bottomrule
\end{tabular}
}
\label{tab:mmscan_caption}
\end{table}

\subsection{Evaluation on 3D Dense Captioning}
\label{sec:dc_results}

3D dense captioning requires the model to localize all the objects in a 3D scene and then generate a descriptive sentence for each object. To evaluate our model on the 3D dense captioning tasks, we utilize the off-the-shelf 3D instance segmentation model~\cite{mask3d} to generate object proposals. Then we further construct the 3D coordinate tokens based on the 3D object center coordinates to guide the model in performing the task. Additionally, we utilize two types of textual instructions that prompt the model to either describe the object or describe and output the bounding box of the object. We report the performance of various methods on two 3D dense captioning benchmarks: Scan2Cap and MMScan Captioning. 

\vspace{3pt}
\noindent\textbf{Scan2Cap.} Scan2Cap requires the model to describe the object's appearance and the spatial relations with nearby objects and output the corresponding 3D bounding box. As illustrated in Tab.~\ref{exp:comparison_on_scanrefer}, our method consistently outperforms the existing method on the Scan2Cap benchmark. 

\vspace{3pt}
\noindent\textbf{MMScan Captioning.} MMScan Captioning focuses on identifying common aspects of 3D objects such as Object Type, Color, Shape, Position, Function, and Design. The benchmark utilizes GPT-4 to assess whether these aspects are correct in the object description compared with the ground truth description. We benchmark various methods on
the MMScan Captioning benchmark in Tab.~\ref{tab:mmscan_caption}. The results show that our method surpasses existing approaches across all metrics by a substantial margin, especially achieving a 49.5\% and 43.3\% improvement in the Color score and the Design score respectively. The strong performance further demonstrates the advantages of architectures based on 2D LMMs.

Uniquely, LLaVA-3D takes multi-view images as inputs, enabling a user-friendly feature where users can simply click on the selected images to generate both 3D object captions and 3D bounding boxes. We refer to this capability as \textit{2D Click-based 3D Dense Captioning}, as illustrated in Fig.~\ref{fig:dense_cap}.


\subsection{Evaluation on 3D Visual Grounding}
\label{sec:vg_results}

3D visual grounding aims to localize the target object in the 3D scene using the natural language description. In this section, we initially report the performance on the ScanRefer~\cite{scanrefer} and Multi3DRef~\cite{zhang2023multi3drefer} benchmarks. For quantitative comparisons, we include both state-of-the-art task-specific models and joint-training 3D LMMs. 3D-LLM~\cite{3dllm} uses the location tokens to discretize the 3D scene and predicts the bounding box as the location tokens that were added to the vocabulary. Chat-3D v2~\cite{chat3d-v2} first segments all the objects and then identify the object that best matches the provided description. The results in Tab.~\ref{tab:vl_results} demonstrate that our LLaVA-3D model achieves promising grounding performance compared to methods that rely on heavy 3D instance segmentation as a prerequisite.

\chenming{we need to emphasize the effectiveness of projected point cloud and reconstruction point cloud.}
%Such a paradigm allows LLaVA-3D to integrate with various powerful 3D grounding modules and inject the 3D understanding capability and world knowledge into the grounding process, as illustrated in Fig.~\ref{fig:demo_2}.%


\begin{table}
\centering
\caption{\textbf{Quantitative comparison with SOTA models on various 3D VG tasks}.}
\vspace{0.1em}
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{lcccc}
    \toprule
     & \multicolumn{2}{c}{ScanRefer} & \multicolumn{2}{c}{Multi3DRef}\\
     \cmidrule(lr){2-3} \cmidrule(lr){4-5}
     & Acc@0.25 & Acc@0.5 & Acc@0.25 & Acc@0.5\\
    \midrule
    \multicolumn{1}{l}{\small\textbf{\textit{Task-specific models}}} \\
    ScanRefer~\cite{scanrefer}	&37.3	&24.3 & - & - 	\\
    MVT~\cite{mvt}	&40.8	&33.3 & - & - \\
    3DVG-Trans~\cite{3dvg-trans} &45.9	&34.5 & - & - \\
    ViL3DRel~\cite{vil3dref}	&47.9	&37.7 & - & - \\  
    BUTD-DETR~\cite{butd-detr}	&52.2 &39.8 & - & - \\  
    ReGround3D~\cite{scanreason}	&\textbf{53.1} &41.1	& - & - \\ 
    M3DRef-CLIP~\cite{scanreason}	&51.0 &\textbf{44.7}	 &42.8 &38.4\\ 
    \midrule
    \multicolumn{1}{l}{\small\textit{\textbf{Joint-Training 3D LMMs}}} \\
    3D-LLM~\cite{3dllm}   	&30.3	&-  &- &- \\
    Chat-3D v2~\cite{chat3d-v2}	&35.9	&30.4  &- &- \\
    Grounded 3D-LLM~\cite{grounded-3d-llm}   &47.9  &44.1 &45.2 &40.6\\ 
    \midrule
    \rowcolor{gray!20} LLaVA-3D	& 51.1 & 41.7 &\textbf{50.1} &\textbf{46.3} \\
    \bottomrule
\end{tabular}
}
\label{tab:vl_results}
\end{table}


\input{figures/dense_cap}

\begin{table}[t!]
\centering
\caption{\textbf{Quantitative Comparisons on zero-shot 2D benchmarks}.}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccccccc}
\toprule
Method & LLM & Res. & {\bf VQA}$^\text{T}$ & {\bf MMB} & {\bf MME} & {\bf MM-Vet} \\
\midrule
MobileVLM~\cite{mobilevlm} & MLLaMA 2.7B & 336 & 47.5  & 59.6 & 1289  &- \\
InstructBLIP~\cite{instructblip} & Vicuna-7B & 224 & 50.1 & 36.0 & -- & 26.2 \\
% InstructBLIP~\cite{instructblip} & Vicuna-13B & 224 & 50.7  & -- & 1213 & 25.6 \\
Qwen-VL~\cite{qwen_vl} & Qwen-7B & 448 & 63.8$^{*}$  & 38.2 & -- & -- \\
Qwen-VL-Chat~\cite{qwen_vl} & Qwen-7B & 448 & 61.5$^{*}$  & 60.6 & 1488  & --   \\
% Shikra~\cite{shikra} & Vicuna-13B & 224 & --  & 58.8 & --  & --  \\
LLaMA-VID~\cite{llama-vid} & Vicuna-7B & 336 & --  & 65.1 & 1521  & -- \\
% LLaMA-VID~\cite{llama-vid} & Vicuna-13B & 336 & -- & 66.6 & 1542  & -- \\
LLaVA-1.5~\cite{llava-1.5} & Vicuna-7B & 336 & 58.2  & 65.2 & 1511  & 31.1  \\
% LLaVA-1.5~\cite{llava-1.5} & Vicuna-13B & 336 & 61.3  & 69.2 & 1531/295  & 36.1 \\
\midrule
\rowcolor{gray!20} LLaVA-3D & Vicuna-7B & 336 & 57.8  & 65.0 & 1502  & 30.9 \\
\bottomrule
\end{tabular}
}
% \vspace{-6mm}
\label{tab:2d_benchmark}
\end{table}

\subsection{Evaluation on 2D benchmarks}
\label{sec:2d_benchmark}

Since our model is trained on the joint 2D and 3D datasets, we evaluate it across various 2D benchmarks to ensure it retains the 2D image understanding capabilities of the original LLaVA. As demonstrated in Tab.~\ref{tab:2d_benchmark}, LLaVA-3D achieves performance comparable to LLaVA-1.5 across various 2D image understanding and conversation benchmarks, which the current existing 3D LMMs do not possess. This performance highlights the architectural advantages of our model over other 3D LMMs.


% \input{figures/visualization}


% \noindent\textbf{Performance on Action tasks}

% To probe LLaVA-3D’s capacity of bridging vision language-acting in the 3D world, we select two canonical
% embodied AI tasks: embodied navigation (ObjNav) on AI
% Habitat and robotic manipulation
% on CLIPort. Specifically, for CLIPort robotic manipulation, we evaluate LLaVA-3D on the three tasks, including their unseen counterparts,
% and report the success scores. For ObjNav, we evaluate
% LLaVA-3D on the original MP3D ObjNav validation split. Aditionally, we test generalization to the validation split of the newly introduced HM3D ObjNav task. We report the success rate and SPL metrics. We consider both
% Habitat-web (fully supervised) and ZSON (zero-shot) as baselines.

% \begin{table}[t]
%     \caption{
%         \textbf{Architecture Comparison} on various 3D V\&L Benchmark.}
%     \centering
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{cccccccc}
%         \toprule
%                & 3D Feature & Connector & LLM / LMM  & ScanQA   & SQA3D  & Inference time \\ 
%         \hline 
%         (a)    & (SAM + CLIP) w / PE & Q-Former & Vicuna-7B & 21.9 & 49.3   & 900s      \\
%         (b)    & (SAM + CLIP) w / PE & Pooling + MLP & Vicuna-7B & 22.1 & 49.2      & 900s \\
%         (c)    & CLIP w / PE   & Pooling + MLP & Vicuna-7B    & 23.4 & 51.2  & 0.2s\\
%         (d)    & CLIP w / PE   & Pooling + MLP  & LLaVA-1.5-7B   & 27.0 & 55.6     & 0.2s \\
%         (e)    & CLIP w / PE   & Pooling + MLP  & PLLaVA-7B~\cite{pllava}       & 27.9 & 56.2  & 0.2s\\ 
%         (f)    & CLIP w / PE   & Pooling + MLP  & InternVL2-7B~\cite{internvl}       & 27.6 & 56.9  & 0.5s\\ 
%         (g)    & CLIP w / PE   & Pooling + MLP  & InternVL2-20B~\cite{internvl}       & 28.1 & 57.1  & 0.5s\\ 
%         \bottomrule
%         \end{tabular}
%     }
%     \label{exp:comparison_on_arch}
% \end{table}

\begin{table*}[t]
    \caption{
        \textbf{Architecture Comparison} on various 3D V\&L Benchmark.}
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{cccccccc}
        \toprule
               & 3D Feature & Connector & LLM / LMM  & ScanQA   & SQA3D  & ScanRefer & Inference time \\ 
        \hline 
        (a)    & (SAM + CLIP) w / PE & Q-Former & Vicuna-7B & 21.9 & 49.3  & - & 900s      \\
        (b)    & (SAM + CLIP) w / PE & Pooling + MLP & Vicuna-7B & 22.1 & 49.2    & - & 900s \\
        (c)    & CLIP w / PE   & Pooling + MLP & Vicuna-7B    & 23.4 & 51.2  & 48.9 & 0.2s\\
        (d)    & CLIP w / PE   & Pooling + MLP  & LLaVA-1.5-7B   & 27.0 & 55.6   & 51.1 & 0.2s \\
        (e)    & CLIP w / PE   & Pooling + MLP  & InternVL2.5-7B~\cite{internvl}       & 28.9 & 58.8 & - & 0.4s\\ 
        \rowcolor{gray!20}(f)    & CLIP w / PE   & Pooling + MLP  & LLaVA-Video-7B~\cite{llava-video}       & \textbf{29.8} & \textbf{60.3} & \textbf{53.2} & 0.4s\\ 
        \bottomrule
        \end{tabular}
    }
    \label{exp:comparison_on_arch}
\end{table*}

% \input{figures/convergene}

\begin{table}[t]
    \caption{
        \textbf{Effectiveness of 3D Patch Representation}. Training using the same instruction tuning datasets, the only difference between multi-image LLaVA and LLaVA-3D is the patch type.}
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{ccccccc}
        \toprule
        Method  & Patch Type  & ScanQA   & SQA3D  & MMScan QA & Scan2Cap \\ \hline
        multi-image LLaVA   & 2D  & 24.1 & 52.3 &  32.7   & 29.1 \\
        \rowcolor{gray!20} LLaVA-3D  & 3D & 27.0 (+2.9) & 55.6 (+3.3) & 41.5 (+8.8)  & 79.2 (+50.1)  \\
        \bottomrule
        \end{tabular}
    }
    \label{tab:3d_patch}
\end{table}


\subsection{Architecture Analysis}
\label{sec:arch_analysis}

In this section, we delve deeper into the architectural benefits and efficacy of adapting a 2D large multimodal model (LMM) to a 3D LMM, as opposed to developing a 3D LMM solely from LLMs. A prominent example of the latter approach is 3D-LLM~\cite{3dllm}, which utilizes established 2D visual foundation models like SAM and CLIP and incorporates 3D multi-view fusion to generate 3D point features, followed by a Q-Former that consolidates these features into a fixed token set.

\vspace{3pt}
\noindent\textbf{Architecture Comparison.} To ensure the fairness of the experiment as much as possible, starting from LLM, we first ablate different 3D feature encoders, and 3D-language connectors using the same instruction tuning datasets. As shown in Tab.~\ref{exp:comparison_on_arch}, the Q-Former (a) and Pooling + MLP (b) share a similar performance on 3D V\&L benchmarks. Notably, using CLIP (c) alone instead of SAM + CLIP (b) achieves better performance and significantly reduces 3D feature extraction computation time from 900s to 0.2s.

\vspace{3pt}
\noindent\textbf{Effectiveness of 3D Patch.} Once we don't decorate the 2D patches with corresponding 3D position embedding, LLaVA-3D will degenerate into 2D multi-image LMMs. To further ascertain the efficacy of our proposed 3D Patch, we conduct additional experiments across a variety of 3D question answering and 3D dense captioning benchmarks. As shown in Tab.~\ref{tab:3d_patch}, integrating 2D patches within a 3D context enhances the model's 3D spatial understanding and reasoning capabilities, resulting in 2.9\% and 3.3\% improvements on the ScanQA and SQA3D benchmarks, respectively. Furthermore, 3D patches prove instrumental in tasks requiring explicit 3D world modeling, yielding substantial performance gains of 8.8\% on the MMScan QA benchmark and a remarkable 50.1\% improvement on the Scan2Cap benchmark.

\vspace{3pt}
\noindent\textbf{Benefits from Video LMMs.} Building upon the established 2D LMMs, our framework substantially benefits from comprehensive pre-training and instruction-tuning on extensive image and video-text datasets. In Tab.~\ref{exp:comparison_on_arch}, we explore the advantages of initializing from a pre-trained 2D LMM (d) compared to starting directly from an LLM (c). Our experimental results consistently show that starting with a well-trained 2D LMM significantly improves performance in 3D spatial understanding tasks. Furthermore, to validate the effectiveness of our method, we adapt LLaVA-3D framework to different video LMMs, such as InternVL2.5~\cite{internvl} and LLaVA-Video~\cite{llava-video}. Furthermore, to validate the effectiveness of our method, we adapt the LLaVA-3D framework to different video LMMs, such as InternVL2.5 and LLaVA-Video, removing the 3D patch pooling process based on their inherently longer context length support. Due to the intrinsic consistency between multi-view image 3D scene representation and video, the results in (e,f) demonstrate that our method can enjoy the significant benefits from video LMMs, especially in 3D question answering tasks. Additionally, we find that initializing from a pre-trained 2D LMM enables LLaVA-3D to achieve a training convergence speed 3.5× faster than that of existing 3D LMMs~\cite{ll3da,leo}. Further details are provided in the supplementary.

\subsection{More Analysis}
\label{sec:ablation}

To better understand the impact of different components of our LLaVA-3D, we conduct a thorough ablation study on the ScanQA and SQA3D benchmarks.

\vspace{3pt}
\noindent\textbf{Impact of Pooling Strategy.} 
% Given the maximum token length limitation of LLMs, we apply pooling to the 3D patch tokens extracted from multi-view images to reduce the number of tokens. However, this pooling process inevitably leads to some information loss. 
Here we conduct various experiments to evaluate the effects of the different pooling strategies. For voxelization pooling, we adopt the simple voxelization approach from ODIN~\cite{odin}. As shown in Tab.~\ref{tab:pooling_strategy}, the voxelization pooling strategy outperforms the FPS pooling method on 3D QA benchmarks. Model performance can be improved by either decreasing voxel size in voxelization pooling or increasing the number of 3D patch tokens in FPS pooling.

\begin{table}
    \caption{
        \textbf{Comparsion on different pooling strategies}.}
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{ccccc}
        \toprule
        Pooling Strategy  & Voxel Size & Token Number & ScanQA   & SQA3D \\ \hline
        Voxelization     & 0.4 & Dynamic        & 24.1 & 53.2                 \\
        Voxelization     & 0.3 & Dynamic        & 25.9 & 54.8               \\
        \rowcolor{gray!20} Voxelization     & 0.2 & Dynamic        & 27.0 & 55.6             \\
        FPS    & -  & 576 & 25.7          & 54.9  \\ 
        FPS     & -  & 1024 & 26.3         & 55.2 \\ 
        \bottomrule
        \end{tabular}
    }
\label{tab:pooling_strategy}
\end{table}

\vspace{3pt}
\noindent\textbf{Multi-View Images Sampling Strategy.} %Due to the redundancy of information among multi-view images and considering computational costs, we sample $V$ views from the egocentric images of the 3D scene in our experiment. In this section, we explore the effect of different image sampling strategies during the inference stage: 1) \textit{Uniform Sampling}: To achieve comprehensive coverage of the entire 3D scene, a straightforward approach is uniform sampling, which samples images evenly. 2) \textit{Text-Guided Sampling}: such sampling strategy uses CLIP to select the frames related to the text instruction during inference based on the image-text CLIP similarity score. Our experiments demonstrate that these two sampling strategies share similar performance on ScanQA and SQA3D, so we choose uniform sampling for simplicity.%
To balance computational efficiency with visual coverage, we sample $V$ views from the egocentric images of each 3D scene. We investigate two sampling strategies during inference: \textit{Uniform Sampling}, which evenly samples images across the scene, and \textit{Text-Guided Sampling}, which selects frames based on CLIP image-text similarity scores to the input instruction. Since our experiments show a similar performance, we adopt uniform sampling for its simplicity.

\vspace{3pt}
\noindent\textbf{Number of Views.} An intuitive assumption is that sampling more views from the 3D scene will preserve more information about the 3D scene. We conduct a comparative experiment varying the number of views sampled from 3D scenes. Tab.~\ref{tab:sample_num} presents the Exact Match (EM) scores on ScanQA and SQA3D across different settings, revealing that the increase in EM score is marginal as the number of views increases. Additionally, the experimental results indicate that exceeding a certain number of views can degrade the model's performance.

\begin{table}
    \caption{
        \textbf{Comparison on performance on 3D QA tasks under different number of multi-view images}.}
    \label{tab:ablation-click-scanqa}
    \centering
    \resizebox{0.95\linewidth}{!}{
        \begin{tabular}{cccc}
        \toprule
        Number of Views  & Number of Tokens & ScanQA   & SQA3D \\ \hline
        16     & 9216         & 26.2 & 55.1              \\
        \rowcolor{gray!20} 20     & 11520         & 27.0 & 55.6             \\
        24     & 13824       & 27.0 & 55.4                 \\
        40     & 23040   &26.7 &55.2  \\ 
        \bottomrule
        \end{tabular}
    }
\label{tab:sample_num}
\end{table}


% \noindent\textbf{Scaling Law for 3D Instruction Tuning.}

% We further conduct an investigation into the scaling law
% regarding different diversities, i.e., scene diversity vs. data sample diversity. The study evaluated the
% performance of the models when subjected to distinct sampling methodologies: uniform sampling of data samples and selective sampling based on scenes (with retention of only samples present within
% the chosen scenes). As depicted in Fig. 9, the performance was found to be relatively lower under
% scenarios with restricted scene diversity, even with an equal distribution of samples. It indicates that
% both data sample and scene diversity matter when scaling up the training and more diverse scenes can
% result in more significant improvement.

% \input{figures/scaling_law}

% \begin{table}
%     \caption{
%         \textbf{Analysis of Scaling Laws with Respect to datasets. The performance is comparatively diminished under conditions where the diversity of the sampled scenes is limited, despite an equivalent allocation of samples.}.}
%     \label{tab:ablation-click-scanqa}
%     \centering
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{ccccc}
%         \toprule
%         Pooling Stratgey  & Voxel Size & Token Number & ScanQA   & SQA3D \\ \hline
%         Voxelization     & 0.18 & Dynamic        & \textbf{13.53} & 15.88                  \\
%         Voxelization     & 0.20 & Dynamic        & \textbf{13.53} & 15.88                  \\
%         Voxelization     & 0.24 & Dynamic        & \textbf{13.53} & 15.88                  \\
%         FPS    & -  & 576 & 11.80          & \textbf{16.74}  \\ 
%         FPS     & -  & 1024 & 11.80          & \textbf{16.74}  \\ 
%         \bottomrule
%         \end{tabular}
%     }
% \end{table}

% \noindent\textbf{Effectiveness of the Base 2D VLM}

% Our model is built on the 2D VLM (LLaVA), which has been consistently updated by the community, like LLaVA-Next, by introducing a high-resolution image encoder and stronger LLM. Here we explore whether our LLaVA-3D model could benefit from stronger base 2D VLM.

% \begin{table}
%     \caption{
%         \textbf{Analysis of Scaling Laws with Base VLM model size.}.}
%     \label{tab:ablation-click-scanqa}
%     \centering
%     \resizebox{0.9\linewidth}{!}{
%         \begin{tabular}{ccccc}
%         \toprule
%         VLM  & LLM  & ScanQA   & SQA3D \\ \hline
%         LLaVA-1.5     & Vicuna-7B        & 24.8   & 54.5               \\
%         LLaVA-1.5     & Vicuna-13B         & 25.1 & 54.9                  \\
%         LLaVA-Next     & Vicuna-7B   & 26.2  & 55.1                 \\
%         LLaVA-Next     & Vicuna-13B     & 26.4 & 55.3                \\
%         LLaVA-Next     & LLaMA3-8B    & - & -               \\
%         \bottomrule
%         \end{tabular}
%     }
% \end{table}

% \noindent\textbf{Effectiveness of 2D/3D Joint Tuning.}

% Since we want to retain the original LMM's 2D image understanding ability, we conduct 2D/3D joint training in the tuning stage. Here we explore the forgetting phenomenon of the large language models during the multi-modal fine-tuning. 






